CollaborER: A Self-supervised Entity Resolution Framework Using Multi-features Collaboration

Entity Resolution (ER) aims to identify whether two tuples refer to the same real-world entity and is well-known to be labor-intensive. It is a prerequisite to anomaly detection, as comparing the attribute values of two matched tuples from two different datasets provides one effective way to detect anomalies. Existing ER approaches, due to insufficient feature discovery or error-prone inherent characteristics, are not able to achieve stable performance. In this paper, we present CollaborER, a self-supervised entity resolution framework via multi-features collaboration. It is capable of (i) obtaining reliable ER results with zero human annotations and (ii) discovering adequate tuples' features in a fault-tolerant manner. CollaborER consists of two phases, i.e., automatic label generation (ALG) and collaborative ER training (CERT). In the first phase, ALG is proposed to generate a set of positive tuple pairs and a set of negative tuple pairs. ALG guarantees the high quality of the generated tuples and hence ensures the training quality of the subsequent CERT. In the second phase, CERT is introduced to learn the matching signals by discovering graph features and sentence features of tuples collaboratively. Extensive experimental results over eight real-world ER benchmarks show that CollaborER outperforms all the existing unsupervised ER approaches and is comparable or even superior to the state-of-the-art supervised ER methods.

==> techniques-old.tex <==
\section{Automatic Label Generation (ALG)}
\label{sec:alg}

In this section, we present an automatic label generation (ALG) strategy.
It contains two components, including (i) a reliable positive label generation (RPLG) method and (ii) a similarity-based negative label generation (SNLG) method.

In general, generating either positive labels or negative labels is highly relevant to the similarity between tuples.
Motivated by the powerful capability of semantics expression of pre-trained language models, we leverage sentence-BERT~\cite{sentenceBERT19}, a variant of BERT that achieves outstanding performance for semantic similarity search, to assign a pre-trained embedding for each tuple.
Then, we use \emph{cosine distance}, a common distance measurement, to quantify the semantic similarity between tuples from different datasets.
The tuple similarity matrix is denoted as $\bm{M_t} \in [0,1]^{|T| \times |T'|}$, where $|T|$ and $|T'|$ represent the total number of tuples in $T$ and $T'$ respectively. In the following, we detail how to generate positive and negative labels via RPLG and SNLG, respectively.

%\vspace{0.05in}
%\noindent
%\textbf
\subsection{Reliable Positive Label Generation (RPLG)}

RPLG aims to find positive candidate tuple pairs with a high probability of being matched.
%Intuitively, if two tuples are matched, they are mutually the most similar to each other.
A common approach is to consider tuples that are mutually most similar to each other.
However, we find empirically many mutually similar tuples do not refer to the same entities.
Considering that high-quality labels are the backbone of the embedding-based ER model as wrong labels will mislead the ER model training, we choose to generate the positive labels by IKGC~\cite{DAT20}, which gives much stronger constraints to ensure the high-quality of positive labels than the methods based on the mutual similarity.
It selects tuple pairs as positive labels that satisfy three requirements~\cite{DAT20}, including (i) both tuples belong to the same positive label; (ii) they are mutually most similar to each other; and (iii) there is a margin between, for each tuple $e$, its most similar tuple and the second most similar one.  
%
%(i) the similarity between the two tuples, which belong to the same positive label, is the highest from both sides; and (ii) there exists a margin between the top-2 candidates.

Specifically, for each tuple $e_i \in T$, we assume that $e_j', e_k' \in T'$ are the tuples that are the most similar and the second most similar tuples in $T'$ to $e_i$, respectively.
%We use $Sim(e_i, e_j')$ to represent the similarity score between $e_i$ and $e_j'$ and use $Sim(e_i, e_k')$ to denote the similarity score between $e_i$ and $e_k'$.
Similarly, for tuple $e_j' \in T'$ (i.e., the most similar tuple to $e_i \in T$), let $e_l$ and $e_u$ denote its most similar tuple in $T$ and second most similar tuple in $T$ respectively. 
%
%, we can compute the similarity score between $e_j'$ and its most similar tuple $e_l$ (w.r.t. is second most similar tuple $e_u$), denoted as $Sim(e_j', e_l)$ (w.r.t. $Sim(e_j', e_u)$).
%
If tuple pair $(e_i, e_j')$ would be considered as a positive label, we expect $e_i = e_l$, i.e., $e_i$ and $e_j'$ are mutually most similar to each, the requirement (ii) stated above. 
%If $e_i = e_l$ (i.e., they are the same tuple) and 
In addition, their similarity discrepancies $\delta_1 = Sim(e_i, e_j') - Sim(e_i, e_k')$ and $\delta_2 = Sim(e_j', e_l) - Sim(e_j', e_u)$ are expected to be both above a given threshold $\theta$, i.e., the requirement (iii) stated above. Here, $Sim(e, e')$ denotes the similarity score between two tuples $e \in T$ and $e'\in T'$. 
%, the tuple pair $(e_i, e_j')$ would be considered as a positive label.

\vspace{0.05in}
\noindent
\textbf{Discussion.}
We would like to emphasize that RPLG is a general approach, which can be easily integrated into various ER methods.
RPLG can not only generate positive labels with high-quality (w.r.t. the experiments to be presented in \textcolor{red}{Section~\ref{exp:ALG_analysis}}) but also achieve desirable ER results without any time-consuming training process (w.r.t. the experiments to be presented in  \textcolor{red}{Section~\ref{sec:ablation}}).

%\vspace{0.05in}
%\noindent
%\textbf
\subsection{Similarity-based Negative Label Generation (SNLG)}

As the random-based negative label generation method has rather limited contribution to the embedding-based ER training, it is essential to generate more ``challenging'' negative labels, as described in Section~\ref{fig:framework}.
To achieve this goal, we propose a similarity-based negative label generation (SNLG) strategy.
Given a positive tuple pair $\mathbb{P}(e_i, e_i')$, where $e_i \in T$ and $e_i' \in T'$, SNLG generates a set of negative labels $\mathbb{N}(e_i, e_i')$ by replacing either $e_i$ or $e_i'$ with its $\epsilon$-nearest neighborhoods in the semantic embedding space.
Again, we use the cosine similarity metric to search for the $\epsilon$-nearest neighbors of $e_i$ and $e_i'$, respectively.

\vspace{0.05in}
\noindent
\textbf{Discussion.}
Though this is a very intuitive and simple method, it effectively promotes the performance of \textsf{CollaborER}.
We will demonstrate the superiority of using the proposed SNLG to generate negative labels for ER in the experiments to be presented in \textcolor{red}{Section~\ref{sec:ablation}}.


\section{Collaborative ER Training (CERT)}
\label{sec:cert}

\begin{figure*}[t]
\centering
\includegraphics[width=7.3in]{table2kg.eps}
% \vspace{-2mm}
\caption{A motivating example of proposing the multi-relational graph construction (MRGC)}
\label{fig:table2kg}
% \vspace*{-2mm}
\end{figure*}

This section introduces a newly proposed collaborative ER training (CERT) approach to discover the features of tuples from both the graph aspect and the sentence aspect to facilitate the ER performance.
CERT is composed of two phases, i.e., (i) multi-relational graph feature learning (MRGFL); and (ii) collaborative sentence feature learning (CSFL).

\subsection{Multi-Relational Graph Feature Learning (MRGFL)}

Inspired by the graph structure's powerful capturing ability of semantics, we propose a multi-relational graph feature learning method (MRGFL) to represent tuples according to their graph features.
It first proposes a \emph{multi-relational graph construction} (MRGC) approach for transforming datasets from the relational format to the graph structure, and then learns the tuple representations via a GNN-based model, e.g., AttrGNN~\cite{AttrGNN20} in our current implementation.


\begin{algorithm}[t]
\LinesNumbered
\DontPrintSemicolon
\caption{Multi-Relational Graph Construction}
\label{algorithm:graph_construction}
    \KwIn{a relational dataset $T$}
    \KwOut{a multi-relational graph $\mathcal{G}$}
    $\mathcal{G} \longleftarrow \varnothing$\;
    \ForEach{$e_i \in T$}{
        $\mathcal{G}$.addNode($e_i$)\;
        \ForEach{$v_j \in \{A_1[e_i], A_2[e_i],...,A_m[e_i]\}$}{
            \If{$v_j$ is not included in $\mathcal{G}$}{
                $\mathcal{G}$.addNode($v_j$)\;
            }
            $r_k \longleftarrow$ find the attribute name of $v_i$\;
            $\mathcal{G}$.addEdge($e_i, r_k, v_j$)\;
        }
    }
\Return{$\mathcal{G}$}
\end{algorithm}

\vspace{0.05in}
\noindent
\textbf{Multi-relational graph construction (MRGC).}
Graph construction techniques have been presented in the existing ER work, such as EMBDI~\cite{CreatingEmDI20} and GraphER~\cite{GraphER20}.
These techniques treat tuples, attribute values, and attribute names as three types of nodes. Edges exist if there are relationships between nodes.
Nonetheless, several drawbacks restrict the scope of using these graph construction methods to perform ER in real-world scenarios.


First, these graph construction approaches may produce intricately large-scale graphs containing a large number of edges and nodes.
Storing a graph with massive edges and nodes is memory-consuming, and meanwhile training a graph embedding model (e.g., GNN) on a large graph is challenging too, as widely-acknowledged by many existing works~\cite{distDGL20, HamiltonYL17, ChenZS18}.
Second, these graph construction methods lack consideration of the semantics contained in an edge itself.
For instance, assume that there are two types edges, i.e., \emph{attribute-value edges} and \emph{tuple-attribute edges}.
The former represents an edge that connects an attribute-level node with a value-level node; the latter represents an edge connecting a tuple-level node with an attribute-level node. 
%a node with the attribute name type and a node with the attribute value type. The latter represents an edge that connects a node with the tuple type and a node with the attribute name type.
%
It is intuitive that these two types of edges have different semantic meanings and hence they should be considered differently when learning features of tuples in the ER task.


The above limitations inspire us to design a relatively \textbf{small-scale} but highly \textbf{effective} MRGC to construct a multi-relational graph for every dataset.
We start by defining a multi-relational graph, formally $\mathcal{G} = \{N, E, A\}$. Here, $N$ and $E$ refer to a set of nodes and edges, respectively; $A$ represents the set of attributes corresponding to the nodes and the edges.
There are two types of nodes in $\mathcal{G}$, i.e., \emph{tuple-level nodes} and \emph{value-level nodes}.
A tuple-level node represents a tuple $e$; while a value-level node corresponds to an attribute value $v$ in a relational dataset.
Each attribute $a \in A$ denotes an attribute name in the relational dataset. 
%\baihua{Is relation a commonly used term? Relation refers to a table in relational databases. Why not use attribute instead?}
${E} = \{(e, a, v) | e, v \in N, a \in A\}$ represents the set of edges.
%, each of which connects a tuple and one of its relevant attribute value.
%
Each edge connects a tuple-level node $e$ to a value-level node $v$ via an attribute $a$, meaning $e$ has $v$ as its value for attribute $a$.

Next, we describe the MRGC procedure, with its pseudo code presented in Algorithm~\ref{algorithm:graph_construction}.
Given a relational dataset $T$, MRGC initializes an empty multi-relational graph $\mathcal{G}$ (Line 1).
Then, MRGC iteratively adds nodes and edges to $\mathcal{G}$ (Lines 2-8).
Specifically, 
for every tuple $e_i\in T$, MRGC first selects its tuple Id as a tuple-level node (Line 3) and then adds a set of value-level nodes that correspond to this tuple (Lines 4-6). Note that, since different tuples share the same attribute names, MRGC generates a set of edges for $e_i$, with each connecting the tuple-level node of $e_i$ and a value-level node $v_j \in \{A_1[e_i], A_2[e_i], \cdots, A_m[e_i]\}$, denoted as $(e_i, a_k, v_j)$.

\vspace{0.05in}
\noindent
\textbf{Discussion.}
Compared to the existing graph construction methods, the proposed MRGC method constructs a small graph that is still able to well preserve the semantics of tuples.
Take the sampled Amazon dataset as an example.
We depict in Figure~\ref{fig:table2kg} the graph structures constructed by three different graph construction methods, including EMBDI~\cite{CreatingEmDI20}, GraphER~\cite{GraphER20}, and the proposed MRGC in this paper.
It is obvious that the graph constructed by MRGC is the smallest, containing fewer nodes and edges than other graphs.
Also, we will verify the small-scale characteristics of MRGC in the experiments to be presented in Section~\textcolor{red}{\ref{exp:HGC_analysis}}.
Besides, MRGC is able to not only preserve the semantic relationships between each tuple and its corresponding attribute values, but also maintain semantic connections between different tuples by connecting them to a shared value-level node.
For example, $e_1$ and $e_2$ have semantic connections since they both have edges linking to the same value-level node ``aspyr media''.

\vspace{0.05in}
\noindent
\textbf{Multi-relational graph feature learning (MRGFL).}
Recall that GNNs-based methods have demonstrated the effectiveness of learning the node embeddings by capturing the graph features, as illustrated in Section~\ref{sec:gnn}. We would like to learn the embeddings of tuples by exploiting a GNN model.
We adopt the state-of-the-art model AttrGNN~\cite{AttrGNN20} for this purpose, since GNNs-based models have been extensively studied.

\textcolor{red}{[cc: I'll re-write this parts as soon as possible.]}
In the following, we illustrate how to exploit AttrGNN to learn tuples' embeddings for ER.
Previous work~\cite{GraphER20, AttrGNN20} suggests that different types of data should be considered differently during embedding learning.
Therefore, we partition the original graph $\mathcal{G}$ generated by MRGC into three disjoint subgraphs, %each of which can be denoted as $\mathcal{G}^{x}$, where $x \in \{1,2,3\}$:
including \emph{name-based graph} $\mathcal{G}^{1}$, \emph{digital-based graph} $\mathcal{G}^{2}$ and \emph{literal-based graph} $\mathcal{G}^{3}$. 
To be more specific, in $\mathcal{G}^{1}$, the value-level nodes only include the values that could almost represent the tuples. \baihua{What do we mean by values that almost represent the tuples? Do you refer to the values of most important attribute?} We find empirically the first column of each row \baihua{This is very ad-hoc. The order of columns in a relation is irrelevant. Why consider the order of the columns instead of the properties of the columns?} can be treated as the tuple's name (e.g., values in the cells of the attribute ``Title'' in the Amazon dataset). 
In $\mathcal{G}^{2}$, the value-level nodes include digits only (e.g., values in the cells of the attribute ``Price'' in the Amazon dataset). \baihua{What are digits? The difference between the digits and values?}
In $\mathcal{G}^{3}$, the value-level nodes include literals only (e.g., values in the cells of the attribute ``Manufacturer'' in the Amazon dataset). \baihua{You only mention value-level nodes here. How about tuple-level nodes? Given a original graph G=\{N, R, E\}, what are the nodes/relations/edges contained by each subgraph? This part is very unclear. }

In each subgraph $\mathcal{G}^{x}$, the embedding of a tuple $e_i$ in $l$-th layer, denoted as $\mathbf{h}_{(e_i,x)}^{l}$, can be learned by AttrGNN as follows:
\begin{equation}
    \mathbf{h}_{(e_i,x)}^{l}=\sigma\left(\sum_{j=1}^{n} \alpha_{j} \mathbf{W}^{l}\left[\mathbf{a}_{j} ; \mathbf{v}_{j}\right]\right)
\end{equation}
where $\sigma$ is the ELU($\cdot$) function, $\alpha_{j}=\frac{\exp \left(o_{j}\right)}{\sum_{k=1}^{n} \exp \left(o_{k}\right)}$, $o_{j}=\operatorname{LeakyReLU}\left(\mathbf{u}^{T}\left[\mathbf{h}_{(e_i,x)}^{l-1} ; \mathbf{a}_{j}\right]\right)$, and $\mathbf{W}$ is a learnable transformation matrix.

The \emph{training objective function} of ER is to unify the two datasets' tuple embeddings generated by each subgraph into a unified semantic vector space by maximizing the similarities with regard to the generated labels.
Formally,
\begin{equation}
    \mathcal{L}_{g}^{x}=\sum_{\left(e_i, e_i'\right) \in \mathbb{P}}\left[d^{x}\!\left(e_i, e_i'\right)^{+} + \gamma - d^{x}\!\left(e_i, e_i'\right)^{-}\right]_{+}
\end{equation}
Here, $(e_i, e_i') \in \mathbb{P}$ represents a positive label; 
$[b]_{+} = max\{0, b\}$;  $d^{x}\!\left(e_i, e_i'\right)^{+}$ denotes the cosine distance between $\boldsymbol{h}_{(e_i,x)}$ and $\boldsymbol{h}_{(e_i',x)}$, where $\boldsymbol{h}_{(e_i,x)}$ and $\boldsymbol{h}_{(e_i',x)}$ are the final embeddings of $e_i$ and $e_i$ w.r.t. the subgraph $\mathcal{G}^{x}$ with $x\in \{1,2,3\}$, after performing the $|l|$ layer AttrGNN model, respectively;
$d^{x}\!\left(e_i, e_i'\right)^{-}$ represents the cosine distance of a negative label belonging to the negative set $\mathbb{N}(e_i, e_i')$; and $\gamma$ is a margin hyper-parameter.

Finally, we can get multiple embeddings of every tuple $e_i$, each of which is derived from a subgraph $G^{x}$.
We ensemble them to obtain a unified embedding of each tuple $e_i$ as follows:
\begin{equation}
    \mathbf{h}_{e_i} = \sum_{x=1}^{3} \beta_{x} \mathbf{h}_{(e_i,x)}
\end{equation}
where $\mathbf{h}_{e_i}$ represents the unified embedding of $e_i$, $\beta_{x} \in [0, 1]$ is a hyper-parameter controlling the contribution of the sentence feature of $e_i$ derived from the subgraph $\mathcal{G}^{x}$. 






\subsection{Collaborative Sentence Feature Learning (CSFL)}

\begin{figure}[t]
\centering
\includegraphics[width=3.65in]{model.eps}
\vspace{-4mm}
\caption{The architecture of CERT}
\label{fig:CSFL_model}
\end{figure}

Recent studies~\cite{Ditto20, AutoEM19, DeepER18} have demonstrated that capturing the sentence features of tuples can help ER task to a certain degree.
Nonetheless, treating tuples as sentences causes insufficient feature discovering, as illustrated in Section~\ref{sec:introduction}.
To this end, we propose a collaborative sentence feature learning (CSFL) model, which discovers sufficient tuples' sentence features for ER with the assistance of the well-trained graph features of tuples.
The training object of CSFL is to (i) identify whether two tuples refer to the same real-world entity; and (ii) minimize the semantic distance between the matched tuples. The architecture of CSFL is depicted in Figure~\ref{fig:CSFL_model}.

First, we present how to identify the matched (or mismatched) tuples in CSFL.
We fine-tune a pre-trained LM with a sentence pair classification task.
We take as inputs a pairwise sentence $\mathcal{S}(e_i, e_i')$ and its corresponding positive and negative labels generated by the proposed ALG.
Then, we learn the classification signal $\rm{\mathbf{E_{[CLS]}}}$ by feeding the inputs into a multi-layer Transformer encoder.
In the current implementation, the number of transformer layers is set to 12, a typical setting used in various tasks.
We use a variant of \emph{CrossEntropy Loss} $\mathcal{L}_1$ as the objective training function, which is derived from Eq.~(\ref{eq:crossentropy_loss}). Formally,
\begin{gather}
\mathcal{L}_1(y=k|\mathcal{S}(e_i, e_i'))  = -\log \left(\frac{\exp (d_k^{*})}{\sum_{j}^{|k|} \exp (d_j^{*})}\right) \forall k \in\{0,1\}\\
\boldsymbol{d}^{*} = \rm{\mathbf{W_c}} \left(\rm{\mathbf{E_{[CLS]}}} ; \rm{\mathbf{G_{abs}}} ; \rm{\mathbf{G_{dot}}} \right)
\end{gather}
Here, the logits $\boldsymbol{d}^{*}$ is produced by both tuples' sentence features (i.e., $\mathbf{E_{[CLS]}}$) and tuples' graph features (i.e., $\mathbf{G_{abs}}$ and $\mathbf{G_{dot}}$).
$\mathbf{G_{abs}} = |\mathbf{h}_{e_i} - \mathbf{h}_{e_i'}|$ denotes the element-wise difference between the graph-based embeddings $\mathbf{h}_{e_i}$ and $\mathbf{h}_{e_i'}$.
$\mathbf{G_{dot}} = \mathbf{h}_{e_i} \otimes \mathbf{h}_{e_i'}$ represents the element-wise similarity between $\mathbf{h}_{e_i}$ and $\mathbf{h}_{e_i'}$.

Second, we illustrate how to minimize the semantic distance between the matched tuples.
At the input, the pre-trained LM allocates an initialized embedding for each token of a sentence $\mathcal{S}(e_i)$ (w.r.t. $\mathcal{S}(e_i')$), denoted as $\rm{\mathbf{E_i}}$ (w.r.t. $\rm{\mathbf{E_i'}}$).
Note that, the special symbol [CLS], which is located in the front of every sentence, also has an initial embedding, denoted as $\rm{\mathbf{E_{[CLS]}}}$.
The embedding of every token will be updated after performing the multi-layer Transformer encoder.
We apply \emph{max-pooling} to obtain a fixed-length embedding $\rm{\mathbf{E_{e_i}}}$ (w.r.t. $\rm{\mathbf{E_{e_i'}}}$) for representing the tuple $e$ (w.r.t. $e'$).
Concretely, max-pooling generates the fixed-length embedding by selecting the maximal value in each dimension among all the embedded tokens of the tuple.
We use \emph{CosineEmbedding Loss} $\mathcal{L}_2$ as the objective training function. It is designed to minimize the semantic distance between matched tuples (w.r.t. the set of positive labels $\mathbb{P}$) and maximize that between mismatched tuples (w.r.t. the set of negative labels $\mathbb{N}$). Formally,
\begin{equation}\label{eq:cosineEmbeddingLoss}
    \mathcal{L}_2(y|\mathcal{S}(e_i), \mathcal{S}(e_j'))=\left\{\begin{array}{ll}
1- \cos (\mathbf{E_{e_i}}, \mathbf{E_{e_j'}}), \text { if } y=1 \\
\max (0, \cos (\mathbf{E_{e_i}}, \mathbf{E_{e_j'}})-\lambda), \text { if } y=0
\end{array}\right.
\end{equation}
where $\lambda$ is a margin hyper-parameter separating matched and mismatched tuple pairs. $\cos (\cdot,\cdot)$ represents the cosine distance metric.

Finally, we are ready to introduce the overall training function of CSFL, namely \emph{collabor training loss} (denoted as $\mathcal{L}_{c}$). Formally,
\begin{equation}
\mathcal{L}_{c} = \mathcal{L}_1 + \mu \mathcal{L}_2
\end{equation}
where hyper-parameter $\mu \in [0,1]$ is a coefficient controlling the relative weight of $\mathcal{L}_2$ against $\mathcal{L}_1$.
The ER results can be obtained according to the predicted labels of each tuple pair.
% First, we describe how CSFL obtains sentence features of tuples.
% Inspired by the success of pre-trained LMs in the ER task, we fine-tune a pre-trained LM for this purpose.
% Given two tuples $e \in T$ and $e' \in T'$, we take three sentences as input, including (i) two serialized tuple $\mathcal{S}(e)$ and $\mathcal{S}(e')$ derived from $e$ and $e'$ respectively; and (ii) one pairwise sentence $\mathcal{S}(e, e')$.





\vspace{0.05in}
\noindent
\textbf{Discussion.}
Compared to the existing sentence-based ER methods that also fine-tune pre-trained LMs, we emphasize the superiority of CSFL in the following two aspects.
First, CSFL incorporates the graph features of tuples learned in the previous MRGFL step to enrich the features that the sentence-based model fails to capture.
Second, we argue that utilizing the CosineEmbedding Loss (i.e., $\mathcal{L}_2$ defined in Equation~\ref{eq:cosineEmbeddingLoss}) as a part of collabor training loss is suitable for the ER task.
Intuitively, matched tuples should have similar embeddings in a unified semantic vector space.
However, the existing sentence-based ER methods, which fine-tune and cast ER
as a sentence-pair classification problem, cannot ensure the semantic similarity between matched tuples.
We will verify the superiority of the proposed CSFL in the experiments to be presented in Section~\ref{sec:ablation}.



